SemEval-2023 Task 12: Sentiment Analysis for African Languages (AfriSenti-SemEval)

We present the first Africentric SemEval Shared task, Sentiment Analysis for African Languages (AfriSenti-SemEval) - The dataset is available at https://github.com/afrisenti-semeval/afrisent-semeval-2023. AfriSenti-SemEval is a sentiment classification challenge in 14 African languages: Amharic, Algerian Arabic, Hausa, Igbo, Kinyarwanda, Moroccan Arabic, Mozambican Portuguese, Nigerian Pidgin, Oromo, Swahili, Tigrinya, Twi, Xitsonga, and Yor\`ub\'a (Muhammad et al., 2023), using data labeled with 3 sentiment classes. We present three subtasks: (1) Task A: monolingual classification, which received 44 submissions; (2) Task B: multilingual classification, which received 32 submissions; and (3) Task C: zero-shot classification, which received 34 submissions. The best performance for tasks A and B was achieved by NLNDE team with 71.31 and 75.06 weighted F1, respectively. UCAS-IIE-NLP achieved the best average score for task C with 58.15 weighted F1. We describe the various approaches adopted by the top 10 systems and their approaches.

==> data_dist.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    language & dpositive & dnegative & dneutral & trpositive & trnegative & trneutral & tepositive & tenegative & teneutral\\
    ary & 385 & 360 & 470 & 1758 & 1664 & 2161 & 1144 & 850 & 967\\
    yor & 884 & 443 & 763 & 3542 & 1872 & 3108 & 1918 & 981 & 1617\\
    tso & 96 & 72 & 35 & 384 & 284 & 136 & 121 & 90 & 43\\
    tir & 61 & 215 & 122 & 0 & 0 & 0 & 643 & 970 & 387\\
    hau & 887 & 894 & 896 & 4687 & 4573 & 4912 & 1755 & 1759 & 1789\\
    twi & 183 & 147 & 58 & 1644 & 1315 & 522 & 450 & 353 & 146\\
    ibo & 560 & 470 & 811 & 3084 & 2600 & 4508 & 1118 & 943 & 1621\\
    swa & 137 & 48 & 268 & 547 & 191 & 1072 & 224 & 80 & 444\\
    kin & 225 & 287 & 315 & 899 & 1146 & 1257 & 278 & 355 & 393\\
    pcm & 447 & 813 & 21 & 1808 & 3421 & 72 & 1397 & 2326 & 431\\
    ama & 333 & 388 & 776 & 1332 & 1548 & 3104 & 438 & 1337 & 224\\
    pt-MZ & 171 & 196 & 400 & 681 & 782 & 1600 & 628 & 655 & 2379\\
    orm & 154 & 117 & 125 & 0 & 0 & 0 & 462 & 733 & 896\\
    arq & 105 & 223 & 86 & 417 & 892 & 342 & 326 & 474 & 154\\
}\devClassDist



\begin{figure}[htp]
    \centering
    \subfloat[Train]{
        \resizebox{\columnwidth}{!}{%
            \begin{tikzpicture}
            \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=5500,        
                ylabel={Number of tweets},
                ylabel near ticks,
                xlabel={Languages},
                xlabel near ticks,
                xtick=data,
                symbolic x coords={ama, arq, ary, hau, ibo, orm, pcm, pt-MZ, kin, swa, tir, tso, twi, yor},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
                ylabel style={font=\fontsize{21}{24}\selectfont},
                xlabel style={font=\fontsize{21}{26}\selectfont},
                legend style={font=\fontsize{21}{26}\selectfont},
                yticklabel style = {font=\huge,xshift=0.5ex},
                xticklabel style = {font=\huge,yshift=0.5ex,rotate=45},
                nodes near coords,  
                every node near coord/.append style={font=\footnotesize, rotate=90, anchor=west},
            ]
            \addplot table[x index=0,y index=4] \devClassDist;
            \addplot table[x index=0,y index=5] \devClassDist;
            \addplot table[x index=0,y index=6] \devClassDist;
        \end{axis}
        \end{tikzpicture}
        }
    }

    \subfloat[Dev]{
        \resizebox{\columnwidth}{!}{%
            \begin{tikzpicture}
            \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=1050,        
                ylabel={Number of tweets},
                ylabel near ticks,
                xlabel={Languages},
                xlabel near ticks,
                xtick=data,
                symbolic x coords={ama, arq, ary, hau, ibo, orm, pcm, pt-MZ, kin, swa, tir, tso, twi, yor},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
                ylabel style={font=\fontsize{21}{24}\selectfont},
                xlabel style={font=\fontsize{21}{26}\selectfont},
                legend style={font=\fontsize{21}{26}\selectfont},
                yticklabel style = {font=\huge,xshift=0.5ex},
                xticklabel style = {font=\huge,yshift=0.5ex,rotate=45},
                nodes near coords,  
                every node near coord/.append style={font=\footnotesize, rotate=90, anchor=west},
            ]
            \addplot table[x index=0,y index=1] \devClassDist;
            \addplot table[x index=0,y index=2] \devClassDist;
            \addplot table[x index=0,y index=3] \devClassDist;
            \end{axis}
            \end{tikzpicture}
        }
    }

    \subfloat[Test]{
        \resizebox{\columnwidth}{!}{%
            \begin{tikzpicture}
            \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=2700,        
                ylabel={Number of tweets},
                ylabel near ticks,
                xlabel={Languages},
                xlabel near ticks,
                xtick=data,
                symbolic x coords={ama, arq, ary, hau, ibo, orm, pcm, pt-MZ, kin, swa, tir, tso, twi, yor},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
                ylabel style={font=\fontsize{21}{24}\selectfont},
                xlabel style={font=\fontsize{21}{26}\selectfont},
                legend style={font=\fontsize{21}{26}\selectfont},
                yticklabel style = {font=\huge,xshift=0.5ex},
                xticklabel style = {font=\huge,yshift=0.5ex,rotate=45},
                nodes near coords,  
                every node near coord/.append style={font=\footnotesize, rotate=90, anchor=west},
            ]
            \addplot table[x index=0,y index=7] \devClassDist;
            \addplot table[x index=0,y index=8] \devClassDist;
            \addplot table[x index=0,y index=9] \devClassDist;
            \end{axis}
            \end{tikzpicture}
        }
    }
    \caption{Datasets Sentiment Class Distribution}
    \label{fig:data_class_dist}
\end{figure}

==> task_a_result.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lrrrrrrrrrrrr}
   \toprule[1.5pt]
         Team & \textbf{\texttt{ama}} & \textbf{\texttt{arq}} & \textbf{\texttt{ary}} & \textbf{\texttt{hau}} & \textbf{\texttt{ibo}} & \textbf{\texttt{kin}} & \textbf{\texttt{pcm}} & \textbf{\texttt{pt-MZ}} & \textbf{\texttt{swa}} & \textbf{\texttt{tso}} & \textbf{\texttt{twi}} & \textbf{\texttt{yor}} \\
    \midrule
        BCAI-AIR3 & 64.04 & 69.99 & \best\textbf{64.83} & \best\textbf{82.62} & \best\textbf{82.96} & \best\textbf{72.63} & 71.94 & 72.90 & \best\textbf{65.68} & \best\textbf{60.67} & 67.51 & 79.95 \\
        PALI & 65.56 & 72.62 & 55.92 & 81.10 & 81.30 & 69.61 & 75.16 & 73.83 & 64.37 & 56.26 & 67.58 & 80.06 \\
        king001 & 69.77 & 73.00 & 57.94 & 81.11 & 81.39 & 60.26 & 75.75 & 73.53 & 64.89 & 56.26 & \best\textbf{68.28} & \best\textbf{80.16} \\
        stce & 65.56 & 71.72 & 55.42 & 80.99 & 81.37 & 69.61 & 75.30 & 73.57 & 64.37 & 56.26 & 67.58 & 80.08 \\
        UM6P & 72.18 & 72.02 & 60.15 & 82.04 & 81.51 & 70.71 & 69.14 & 67.35 & 60.26 & 56.13 & 66.98 & 76.01 \\
        mitchelldehaven & 60.83 & 69.64 & 63.54 & 78.75 & 78.99 & 72.48 & 69.17 & 72.28 & 63.01 & 60.32 & 65.98 & 77.25 \\
        ymf924 & 69.83 & 67.83 & 57.12 & 75.88 & 72.49 & 70.88 & 72.48 & 73.80 & 64.23 & 55.38 & 62.56 & 75.94 \\
        NLP-LISAC & 64.71 & \best\textbf{74.20} & 62.11 & 79.74 & 79.66 & 65.59 & 68.00 & 65.90 & 59.69 & 53.72 & 66.38 & 75.42 \\
        GMNLP & \best\textbf{78.42} & 67.99 & 55.23 & 79.56 & 75.34 & 71.80 & 68.84 & 71.90 & 63.70 & 51.67 & 56.46 & 70.84 \\
        ABCD Team & 58.05 & 63.50 & 61.54 & 81.50 & 82.28 & 67.36 & 66.30 & 67.21 & 63.10 & 53.92 & 65.61 & 79.73 \\
        tmn & 63.11 & 70.54 & 57.22 & 72.93 & 72.66 & 69.82 & 69.63 & 73.09 & 61.66 & 53.66 & 67.06 & 75.08 \\
        PA14 & 64.52 & 72.01 & 55.34 & 77.17 & 80.29 & 61.16 & 75.53 & \best\textbf{74.98} & 61.73 & 50.46 & 67.39 & 65.65 \\
        UCAS-IIE-NLP & 67.45 & 63.31 & 55.36 & 80.79 & 78.51 & 71.47 & 66.63 & 65.13 & 60.73 & 51.09 & 60.15 & 77.13 \\
        HausaNLP & 57.30 & 65.12 & 58.49 & 80.97 & 76.96 & 70.61 & 68.48 & 68.37 & 63.23 & 50.27 & 64.07 & 71.88 \\
        UIO & 56.86 & 69.21 & 57.46 & 74.63 & 77.58 & 61.66 & 67.08 & 71.64 & 56.69 & 60.07 & 65.02 & 66.99 \\
        Masakhane-Afrisenti & 68.85 & 64.35 & 55.50 & 73.12 & 73.75 & 64.14 & 66.88 & 70.26 & 60.24 & 54.33 & 62.83 & 68.98 \\
        DN & 57.34 & 65.81 & 57.20 & 81.09 & 74.51 & 71.91 & 64.89 & 69.09 & 62.51 & 46.62 & 55.53 & 72.07 \\
        UMUTeam & 55.39 & 68.52 & 54.75 & 73.92 & 76.78 & 65.03 & 65.55 & 71.14 & 60.52 & 54.89 & 63.01 & 66.10 \\
        Howard University CS & 61.68 & 62.49 & 47.34 & 77.68 & 78.02 & 66.50 & 66.12 & 67.72 & 52.31 & 48.80 & 62.84 & 74.72 \\
        FIT BUT & 65.10 & 62.15 & 52.08 & 72.56 & 75.64 & 67.25 & 65.00 & 63.54 & 57.90 & 52.86 & 63.41 & 67.93 \\
        UBC-DLNLP & 56.88 & 64.02 & 53.06 & 79.37 & 77.52 & 62.02 & 65.57 & 61.98 & 58.60 & 45.49 & 65.14 & 71.02 \\
        Witcherses & 39.09 & 57.55 & 50.68 & 79.65 & 80.87 & 62.69 & 64.44 & 65.03 & 58.91 & 52.82 & 66.47 & 78.44 \\
        Sefamerve & 70.18 & 71.74 & 52.54 & 78.59 & 73.24 & 63.15 & 63.67 & 67.94 & 63.94 & 48.27 & 65.66 & 25.33 \\
        FUOYENLP & 54.25 & 68.14 & 52.78 & 73.17 & 72.22 & 54.20 & 68.01 & 72.88 & 54.31 & 51.38 & 57.94 & 64.31 \\
        efrat4050 & 31.99 & 55.40 & 54.43 & 75.65 & 76.28 & 59.56 & 53.17 & 62.75 & 51.76 & 54.10 & 64.18 & 72.76 \\
        JCT & 53.76 & 24.59 & 43.95 & 79.50 & 77.08 & 58.22 & 62.52 & 62.96 & 58.98 & 54.10 & 61.82 & 69.98 \\
        JacobLevy248 & 21.55 & 54.71 & 46.32 & 73.38 & 78.14 & 57.92 & 57.47 & 62.67 & 55.97 & 51.26 & 64.06 & 64.83 \\
        jacklight971 & 53.76 & 24.59 & 43.95 & 79.57 & 75.79 & 51.41 & 62.17 & 55.65 & 58.98 & 42.74 & 60.37 & 63.96 \\
        MaChAmp & 2.26 & 32.87 & 12.79 & 17.02 & 26.91 & 17.79 & 40.20 & 51.17 & 44.22 & 26.01 & 20.17 & 18.87 \\\hline
        TechSSN & - & - & - & 80.32 & - & - & - & - & - & - & - & - \\
        KINLP & - & - & - & - & - & 72.50 & - & - & - & - & - & - \\
        afrisenti23kb & - & - & - & - & - & 71.00 & - & - & - & - & - & - \\
        foul & - & 70.36 & - & - & - & - & - & - & - & - & - & - \\
        Bhattacharya\_Lab & - & - & - & - & - & 47.10 & \best\textbf{75.96} & - & - & - & - & 79.86 \\
        uid & - & - & 55.29 & 80.45 & 78.51 & 70.99 & - & - & - & 46.91 & 59.63 & 76.98 \\
        TBS & - & - & 55.29 & 80.67 & 78.47 & 70.98 & - & - & - & 49.40 & 55.11 & 76.57 \\
        DuluthNLP & - & - & - & - & - & - & 65.85 & - & - & - & 64.29 & - \\
        akn & - & - & - & - & - & - & 64.69 & - & - & - & - & - \\
        Seals\_Lab & 54.67 & - & - & 80.85 & 80.82 & - & - & 52.43 & 52.18 & - & - & - \\
        NLP-LTU & - & - & 60.27 & - & - & - & - & - & - & - & - & - \\
        Trinity & - & - & - & 76.53 & - & - & - & - & 47.55 & - & - & 50.00 \\
        ronaharo & 14.98 & - & 39.72 & 72.84 & 73.21 & 57.87 & 62.52 & 53.35 & - & - & - & - \\
        GunadarmaxBRIN & - & - & - & - & - & - & - & - & - & 50.11 & - & - \\
        aptxaaaa & - & - & 51.01 & - & - & - & - & - & - & 48.97 & - & - \\
    \bottomrule
    \end{tabular}
    }
    \caption{Task A Results.}
    \label{tab:task_a_results}
\end{table*}




% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{clrrrrrrrrrrrrr}
%    \toprule[1.5pt]
%          \# & Team & \textbf{\texttt{ama}} & \textbf{\texttt{arq}} & \textbf{\texttt{ary}} & \textbf{\texttt{hau}} & \textbf{\texttt{ibo}} & \textbf{\texttt{kin}} & \textbf{\texttt{pcm}} & \textbf{\texttt{pt-MZ}} & \textbf{\texttt{swa}} & \textbf{\texttt{tso}} & \textbf{\texttt{twi}} & \textbf{\texttt{yor}} & \textbf{Avg.}\\
%     \midrule
%         \textbf{1} & BCAI-AIR3 & 64.04 & 69.99 & \best\textbf{64.83} & \best\textbf{82.62} & \best\textbf{82.96} & \best\textbf{72.63} & 71.94 & 72.90 & \best\textbf{65.68} & \best\textbf{60.67} & 67.51 & 79.95 & \best\textbf{71.31} \\
%         \textbf{2} & PALI & 65.56 & 72.62 & 55.92 & 81.10 & 81.30 & 69.61 & 75.16 & 73.83 & 64.37 & 56.26 & 67.58 & 80.06 & 70.28 \\
%         \textbf{3} & king001 & 69.77 & 73.00 & 57.94 & 81.11 & 81.39 & 60.26 & 75.75 & 73.53 & 64.89 & 56.26 & \best\textbf{68.28} & \best\textbf{80.16} & 70.20 \\
%         \textbf{4} & stce & 65.56 & 71.72 & 55.42 & 80.99 & 81.37 & 69.61 & 75.30 & 73.57 & 64.37 & 56.26 & 67.58 & 80.08 & 70.15 \\
%         \textbf{5} & UM6P & 72.18 & 72.02 & 60.15 & 82.04 & 81.51 & 70.71 & 69.14 & 67.35 & 60.26 & 56.13 & 66.98 & 76.01 & 69.54 \\
%         \textbf{6} & mitchelldehaven & 60.83 & 69.64 & 63.54 & 78.75 & 78.99 & 72.48 & 69.17 & 72.28 & 63.01 & 60.32 & 65.98 & 77.25 & 69.35 \\
%         \textbf{7} & ymf924 & 69.83 & 67.83 & 57.12 & 75.88 & 72.49 & 70.88 & 72.48 & 73.80 & 64.23 & 55.38 & 62.56 & 75.94 & 68.20 \\
%         \textbf{8} & NLP-LISAC & 64.71 & \best\textbf{74.20} & 62.11 & 79.74 & 79.66 & 65.59 & 68.00 & 65.90 & 59.69 & 53.72 & 66.38 & 75.42 & 67.93 \\
%         \textbf{9} & GMNLP & \best\textbf{78.42} & 67.99 & 55.23 & 79.56 & 75.34 & 71.80 & 68.84 & 71.90 & 63.70 & 51.67 & 56.46 & 70.84 & 67.65 \\
%         \textbf{10} & ABCD Team & 58.05 & 63.50 & 61.54 & 81.50 & 82.28 & 67.36 & 66.30 & 67.21 & 63.10 & 53.92 & 65.61 & 79.73 & 67.51 \\
%         \textbf{11} & tmn & 63.11 & 70.54 & 57.22 & 72.93 & 72.66 & 69.82 & 69.63 & 73.09 & 61.66 & 53.66 & 67.06 & 75.08 & 67.21 \\
%         \textbf{12} & PA14 & 64.52 & 72.01 & 55.34 & 77.17 & 80.29 & 61.16 & 75.53 & \best\textbf{74.98} & 61.73 & 50.46 & 67.39 & 65.65 & 67.19 \\
%         \textbf{13} & UCAS-IIE-NLP & 67.45 & 63.31 & 55.36 & 80.79 & 78.51 & 71.47 & 66.63 & 65.13 & 60.73 & 51.09 & 60.15 & 77.13 & 66.48 \\
%         \textbf{14} & HausaNLP & 57.30 & 65.12 & 58.49 & 80.97 & 76.96 & 70.61 & 68.48 & 68.37 & 63.23 & 50.27 & 64.07 & 71.88 & 66.31 \\
%         \textbf{15} & UIO & 56.86 & 69.21 & 57.46 & 74.63 & 77.58 & 61.66 & 67.08 & 71.64 & 56.69 & 60.07 & 65.02 & 66.99 & 65.41 \\
%         \textbf{16} & Masakhane-Afrisenti & 68.85 & 64.35 & 55.50 & 73.12 & 73.75 & 64.14 & 66.88 & 70.26 & 60.24 & 54.33 & 62.83 & 68.98 & 65.27 \\
%         \textbf{17} & DN & 57.34 & 65.81 & 57.20 & 81.09 & 74.51 & 71.91 & 64.89 & 69.09 & 62.51 & 46.62 & 55.53 & 72.07 & 64.88 \\
%         \textbf{18} & UMUTeam & 55.39 & 68.52 & 54.75 & 73.92 & 76.78 & 65.03 & 65.55 & 71.14 & 60.52 & 54.89 & 63.01 & 66.10 & 64.63 \\
%         \textbf{19} & Howard University CS & 61.68 & 62.49 & 47.34 & 77.68 & 78.02 & 66.50 & 66.12 & 67.72 & 52.31 & 48.80 & 62.84 & 74.72 & 63.85 \\
%         \textbf{20} & FIT BUT & 65.10 & 62.15 & 52.08 & 72.56 & 75.64 & 67.25 & 65.00 & 63.54 & 57.90 & 52.86 & 63.41 & 67.93 & 63.79 \\
%         \textbf{21} & UBC-DLNLP & 56.88 & 64.02 & 53.06 & 79.37 & 77.52 & 62.02 & 65.57 & 61.98 & 58.60 & 45.49 & 65.14 & 71.02 & 63.39 \\
%         \textbf{22} & Witcherses & 39.09 & 57.55 & 50.68 & 79.65 & 80.87 & 62.69 & 64.44 & 65.03 & 58.91 & 52.82 & 66.47 & 78.44 & 63.05 \\
%         \textbf{23} & Sefamerve & 70.18 & 71.74 & 52.54 & 78.59 & 73.24 & 63.15 & 63.67 & 67.94 & 63.94 & 48.27 & 65.66 & 25.33 & 62.02 \\
%         \textbf{24} & FUOYENLP & 54.25 & 68.14 & 52.78 & 73.17 & 72.22 & 54.20 & 68.01 & 72.88 & 54.31 & 51.38 & 57.94 & 64.31 & 61.97 \\
%         \textbf{25} & efrat4050 & 31.99 & 55.40 & 54.43 & 75.65 & 76.28 & 59.56 & 53.17 & 62.75 & 51.76 & 54.10 & 64.18 & 72.76 & 59.34 \\
%         \textbf{26} & JCT & 53.76 & 24.59 & 43.95 & 79.50 & 77.08 & 58.22 & 62.52 & 62.96 & 58.98 & 54.10 & 61.82 & 69.98 & 58.96 \\
%         \textbf{27} & JacobLevy248 & 21.55 & 54.71 & 46.32 & 73.38 & 78.14 & 57.92 & 57.47 & 62.67 & 55.97 & 51.26 & 64.06 & 64.83 & 57.36 \\
%         \textbf{28} & jacklight971 & 53.76 & 24.59 & 43.95 & 79.57 & 75.79 & 51.41 & 62.17 & 55.65 & 58.98 & 42.74 & 60.37 & 63.96 & 56.08 \\
%         \textbf{29} & MaChAmp & 2.26 & 32.87 & 12.79 & 17.02 & 26.91 & 17.79 & 40.20 & 51.17 & 44.22 & 26.01 & 20.17 & 18.87 & 25.86 \\\hline
%         \textbf{NR} & TechSSN & - & - & - & 80.32 & - & - & - & - & - & - & - & - & 80.32 \\
%         \textbf{NR} & KINLP & - & - & - & - & - & 72.50 & - & - & - & - & - & - & 72.50 \\
%         \textbf{NR} & afrisenti23kb & - & - & - & - & - & 71.00 & - & - & - & - & - & - & 71.00 \\
%         \textbf{NR} & foul & - & 70.36 & - & - & - & - & - & - & - & - & - & - & 70.36 \\
%         \textbf{NR} & Bhattacharya\_Lab & - & - & - & - & - & 47.10 & \best\textbf{75.96} & - & - & - & - & 79.86 & 67.64 \\
%         \textbf{NR} & uid & - & - & 55.29 & 80.45 & 78.51 & 70.99 & - & - & - & 46.91 & 59.63 & 76.98 & 66.97 \\
%         \textbf{NR} & TBS & - & - & 55.29 & 80.67 & 78.47 & 70.98 & - & - & - & 49.40 & 55.11 & 76.57 & 66.64 \\
%         \textbf{NR} & DuluthNLP & - & - & - & - & - & - & 65.85 & - & - & - & 64.29 & - & 65.07 \\
%         \textbf{NR} & akn & - & - & - & - & - & - & 64.69 & - & - & - & - & - & 64.69 \\
%         \textbf{NR} & Seals\_Lab & 54.67 & - & - & 80.85 & 80.82 & - & - & 52.43 & 52.18 & - & - & - & 64.19 \\
%         \textbf{NR} & NLP-LTU & - & - & 60.27 & - & - & - & - & - & - & - & - & - & 60.27 \\
%         \textbf{NR} & Trinity & - & - & - & 76.53 & - & - & - & - & 47.55 & - & - & 50.00 & 58.03 \\
%         \textbf{NR} & ronaharo & 14.98 & - & 39.72 & 72.84 & 73.21 & 57.87 & 62.52 & 53.35 & - & - & - & - & 53.50 \\
%         \textbf{NR} & GunadarmaxBRIN & - & - & - & - & - & - & - & - & - & 50.11 & - & - & 50.11 \\
%         \textbf{NR} & aptxaaaa & - & - & 51.01 & - & - & - & - & - & - & 48.97 & - & - & 49.99 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Task A Results. Ranking based on average of the scores. Partial submissions are not included in the final ranking. \textbf{NR} - No Ranking.}
%     \label{tab:task_a_results}
% \end{table*}
